Randomized Dimensionality Reduction for k-means Clustering

We study the topic of dimensionality reduction for $k$-means clustering. Dimensionality reduction encompasses the union of two approaches: \emph{feature selection} and \emph{feature extraction}. A feature selection based algorithm for $k$-means clustering selects a small subset of the input features and then applies $k$-means clustering on the selected features. A feature extraction based algorithm for $k$-means clustering constructs a small set of new artificial features and then applies $k$-means clustering on the constructed features. Despite the significance of $k$-means clustering as well as the wealth of heuristic methods addressing it, provably accurate feature selection methods for $k$-means clustering are not known. On the other hand, two provably accurate feature extraction methods for $k$-means clustering are known in the literature; one is based on random projections and the other is based on the singular value decomposition (SVD). This paper makes further progress towards a better understanding of dimensionality reduction for $k$-means clustering. Namely, we present the first provably accurate feature selection method for $k$-means clustering and, in addition, we present two feature extraction methods. The first feature extraction method is based on random projections and it improves upon the existing results in terms of time complexity and number of features needed to be extracted. The second feature extraction method is based on fast approximate SVD factorizations and it also improves upon the existing results in terms of time complexity. The proposed algorithms are randomized and provide constant-factor approximation guarantees with respect to the optimal $k$-means objective value.

==> bio.tex <==

Christos Boutsidis is a Research Scientist at Yahoo Labs in New York, NY. 
Before that he was a Research Staff Member at the Business Analytics and Mathematical Sciences Department of the IBM T.J Watson 
Research Center in Yorktown Heights, NY. Dr Boutsidis earned a Ph.D. in Computer Science from Rensselaer Polytechnic Institute in 
May of 2011 and a BS in Computer Engineering and Informatics from the University of Patras, Greece in July of 2006. Dr Boutsidis' research 
interests lie in the design and analysis of fast approximation algorithms for matrix computations and applications of those to machine 
learning and data analysis problems. Dr Boutsidis has published over 25 articles in conferences and journals in numerical linear algebra,
theoretical computer science, and statistical data analysis. 

Anastasios Zouzias received his M.Sc. degree and Ph.D. degree in computer science from the University of Toronto, Canada, in 2009 and 2013, respectively. Currently, he has been with IBM Research Zurich, Switzerland, where he is a post-doctoral research scientist. His research interests include information retrieval, machine learning, randomized approximation algorithms, and randomized algorithms for numerical linear algebra.

Michael Mahoney is at the University of California at Berkeley in the 
Department of Statistics and at the International Computer Science 
Institute.  He works on algorithmic and statistical aspects of modern 
large-scale data analysis.  Much of his recent research has focused on 
large-scale machine learning, including randomized matrix algorithms and 
randomized numerical linear algebra, geometric network analysis tools for 
structure extraction in large informatics graphs, scalable implicit 
regularization methods, and applications in genetics, astronomy, medical 
imaging, social network analysis, and internet data analysis.  He received 
him PhD from Yale University with a dissertation in computational 
statistical mechanics, and he has worked and taught at Yale University in 
the mathematics department, at Yahoo Research, and at Stanford University 
in the mathematics department.  Among other things, he is on the national 
advisory committee of the Statistical and Applied Mathematical Sciences 
Institute (SAMSI), he was on the National Research Council's Committee on 
the Analysis of Massive Data, he runs the biennial MMDS Workshops on 
Algorithms for Modern Massive Data Sets, and he spent fall 2013 at UC 
Berkeley co-organizing the Simons Foundation's program on the Theoretical 
Foundations of Big Data Analysis.


Prof. Drineas is an Associate Professor at the Computer Science Department of Rensselaer Polytechnic
Institute. Prof. Drineas earned a PhD in Computer Science from Yale University in May of 2003, and a 
BS in Computer Engineering and Informatics from the University of Patras, Greece, in July of 1997. Prof. 
Drineas' research interests lie in the design and analysis of randomized algorithms for linear algebraic 
problems, as well as their applications to the analysis of modern, massive datasets. Prof. Drineas was 
a Visiting Professor at the US Sandia National Laboratories during the fall of 2005, a Visiting Fellow at 
the Institute for Pure and Applied Mathematics at the University of California, Los Angeles in the fall of 
2007, and a Visiting Professor at the University of California Berkeley in the fall of 2013. Prof. Drineas 
has also served the US National Science Foundation (NSF) as a Program Director in the Information and 
Intelligent Systems (IIS) Division and the Computing and Communication Foundations (CCF) Division 
(2010-2011). Prof. Drineas has published over 90 articles in conferences and journals in Theoretical 
Computer Science, Numerical Linear Algebra, and statistical data analysis.
